How Trustworthy are Open-Source LLMs? An Assessment under Malicious Demonstrations Shows their Vulnerabilities

The rapid progress in open-source Large Language Models (LLMs) is significantly driving AI development forward. However, there is still a limited understanding of their trustworthiness. Deploying these models at scale without sufficient trustworthiness can pose significant risks, highlighting the need to uncover these issues promptly. In this work, we conduct an adversarial assessment of open-source LLMs on trustworthiness, scrutinizing them across eight different aspects including toxicity, stereotypes, ethics, hallucination, fairness, sycophancy, privacy, and robustness against adversarial demonstrations. We propose advCoU, an extended Chain of Utterances-based (CoU) prompting strategy by incorporating carefully crafted malicious demonstrations for trustworthiness attack. Our extensive experiments encompass recent and representative series of open-source LLMs, including Vicuna, MPT, Falcon, Mistral, and Llama 2. The empirical outcomes underscore the efficacy of our attack strategy across diverse aspects. More interestingly, our result analysis reveals that models with superior performance in general NLP tasks do not always have greater trustworthiness; in fact, larger models can be more vulnerable to attacks. Additionally, models that have undergone instruction tuning, focusing on instruction following, tend to be more susceptible, although fine-tuning LLMs for safety alignment proves effective in mitigating adversarial trustworthiness attacks.

==> figures/result_base.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/base.pdf}
    \caption{Results for the base version of five series of LLMs with different model sizes.}
    \label{result_base}
\end{figure}

==> figures/result_base_2.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/base_2.pdf}
    \caption{Average ASR scores across eight trustworthiness aspects for base models in five LLM series with varying model sizes. We find that the \textsc{Llama 2} series exhibits the highest attack success rates, despite being known as the strongest among those five for general NLP tasks.}
    \label{result_base_2}
\end{figure}

==> tables/models.tex <==

\begin{table*}[htbp]
\centering
\caption{Candidate Models.}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|c|ccc}
\toprule
\textbf{Model} & \textbf{Variant} & Release Time & Size & Base Model   \\
\midrule

\multirow{3}{*}{\textbf{Vacuna}} & Vacuna-7B & \multirow{3}{*}{Mar-2023}  & 7B & \multirow{3}{*}{LLaMA}  \\
 & Vacuna-13B &  & 13B &  \\ 
  & Vacuna-33B &  & 33B &  \\ 
 \midrule

\multirow{3}{*}{\textbf{LLaMA 2}} & LLaMA-2-7B-Chat & \multirow{3}{*}{Jul-2023}  & 7B & \multirow{3}{*}{LLaMA} \\
& LLaMA-2-13B-Chat &  & 13B &  \\ 
& LLaMA-2-70B-Chat &  & 70B &  \\ 
 \midrule

\multirow{1}{*}{\textbf{Alpaca}} & Alpaca-7B & Mar-2023  & 7B & LLaMA  \\
\midrule

\multirow{2}{*}{\textbf{Pythia}} & Pythia-6.9B & \multirow{2}{*}{Apr-2023} & 6.9B & \multirow{2}{*}{-}  \\
& Pythia-12B &  & 12B &  \\ 
 \midrule

\multirow{2}{*}{\textbf{MPT}} & MPT-7B-Chat &  \multirow{2}{*}{May-2023}  & 7B & \multirow{2}{*}{-}  \\
 & MPT-30B-Chat &  & 30B &  \\ 
 \midrule

\multirow{2}{*}{\textbf{Falcon}} & Falcon-7B-instruct & \multirow{2}{*}{May-2023}  & 7B & \multirow{2}{*}{-}  \\
 & Falcon-40B-instruct &  & 40B &  \\ 
 \midrule


\bottomrule
\end{tabular}
}
\label{tab:model_list}
\end{table*}

==> tables/results_1.tex <==
\begin{table*}[htbp]
\centering
\caption{Experimental results for different trustworthiness aspects. We use the toxicity score generated by the Perspective API as the metric for ``Toxicity'' and employ the attack success rate (ASR) for other aspects}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|ccc|cc|cc|c|ccc}
\toprule
\multirow{2}{*}{\textbf{Aspect}} & \multirow{2}{*}{\textbf{Method}} &  \multicolumn{3}{c|}{Vicuna-v1.3}  & \multicolumn{2}{c|}{MPT (Base)} & \multicolumn{2}{c|}{Falcon (Base)}& \multicolumn{1}{c|}{Mistral (Base)} & \multicolumn{3}{c}{Llama 2 (Base)}    \\
& & 7B & 13B & 33B & 7B & 30B & 7B & 40B & 7B & 7B & 13B & 70B  \\
\midrule
\multirow{2}{*}{\textbf{Toxicity}} & DT  & 0.37  & 0.33 & 0.70  &  0.27 & 0.30  & 0.20 & 0.29 & 0.41 & 0.18 & 0.29 & 0.43    \\
 & Ours  & 0.80  & 0.78  & 0.76 & 0.28  & 0.77  & 
 0.25 & 0.75 & 0.79  & 0.83   & 0.78  &  0.74  \\ \midrule

\multirow{2}{*}{\textbf{Stereotype}} & DT  & 1.2\%  & 90.9\% & 2.0\%  & 100.0\% & 99.5\% & 99.9\% & 91.8\% &  100.0\% & 100.0\%  & 100.0\%  &  100.0\%  \\
& Ours  & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\% &  100.0\%  \\ \midrule

\multirow{2}{*}{\textbf{Ethics}} & DT  &  45.6\% & 88.7\%  & 100.0\%  & 63.6\% & 87.9\% & 81.4\% & 82.5\% & 37.5\%  & 42.5\%  & 33.0\% & 3.1\%    \\
& Ours  & 41.6\% & 100.0\%  & 100.0\%  & 100.0\% & 100.0\% & 100.0\%  &  100.0\% & 100.0\%  & 100.0\%  & 100.0\% & 100.0\%   \\ \midrule

\multirow{2}{*}{\textbf{Hallucination}} & DT  & - & - & - & - & - & - & - & - & - & - & -    \\
& Ours  & 0.4\%  & 6.8\%  & 57.2\%  & 0.1\%  & 70.5\% & 9.3\% & 6.7\% & 72.9\%  & 54.9\% & 50.9\%  & 99.8\%   \\ \midrule

\multirow{2}{*}{\textbf{Fairness}} & DT  & 46.0\%  & 41.0\% & 27.0\%  & 50.0\% & 53.0\% & 50.0\% & 42.0\% & 37.0\% & 46.0\% & 44.0\% & 27.0\%    \\
& Ours  & 50.0\%  & 50.0\%  & 50.0\%  & 50.0\% & 51.0\% & 50.0\% & 50.0\% & 50.0\%  & 62.0\%  & 87.0\%  &  61.0\%  \\ \midrule

\multirow{2}{*}{\textbf{Sycophancy}} & DT  & -  & -  & -  & - & - & - & -  & - & - & - & -    \\
& Ours  & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ \midrule

\multirow{2}{*}{\textbf{Privacy}} & DT  &  99.2\% & 98.3\% & 99.8\% & 100.0\% & 100.0\% & 99.9\% & 100.0\% & 99.9\% & 100.0\% & 99.9\%  & 99.9\%    \\
& Ours  & 99.6\% & 99.7\%  & 99.8\%  & 100.0\% & 100.0\% & 99.9\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ \midrule

\multirow{2}{*}{\textbf{Robustness}} & DT  & 26.6\%  & 34.1\%  & 12.8\%  & 49.4\% & 56.6\% & 63.5\% & 28.8\% & 53.6\% & 47.9\% & 51.9\% & 42.0\%    \\
& Ours  & 97.4\%  & 100.0\%  & 100.0\%  & 98.8\% & 98.6\% & 89.5\% & 88.8\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ 

\bottomrule
\end{tabular}
}
\label{tab:results_1}
\end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Experimental results for different trustworthiness aspects. We use the toxicity score generated by the Perspective API as the metric for ``Toxicity'' and employ the attack success rate (ASR) for other aspects}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lc|ccc|cc|cc|c|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Aspect}} & \multirow{2}{*}{\textbf{Method}} &  \multicolumn{3}{c|}{Vicuna-v1.3}  & \multicolumn{2}{c|}{MPT (Base)} & \multicolumn{2}{c|}{Falcon (Base)}& \multicolumn{1}{c|}{Mistral (Base)} & \multicolumn{3}{c}{Llama 2 (Base)}    \\
% & & 7B & 13B & 33B & 7B & 30B & 7B & 40B & 7B & 7B & 13B & 70B  \\
% \midrule
% \multirow{2}{*}{\textbf{Toxicity}} & DT  &   &  &   &  &  & &  &  &  &  &     \\
%  & Ours  & 0.80  & 0.78  & 0.76 & 0.28 & 0.77  & 0.25 & 0.75 & 0.79  & 0.83   & 0.78  &  0.74  \\ \midrule

% \multirow{2}{*}{\textbf{Stereotype}} & DT  &   &  &   &  &  & &  &   &   &   &    \\
% & Ours  & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\% &  100.0\%  \\ \midrule

% \multirow{2}{*}{\textbf{Ethics}} & DT  &   &   &   &  &  & &  &   &   &  &     \\
% & Ours  & 41.6\% & 100.0\%  & 100.0\%  & 100.0\% & 100.0\% & 100.0\% &  100.0\% & 100.0\%  & 100.0\%  & 100.0\% & 100.0\%   \\ \midrule

% \multirow{2}{*}{\textbf{Hallucination}} & DT  &  &  &  &  &  & &  &  &  &  &     \\
% & Ours  & 0.4\%  & 6.8\%  & 57.2\%  & 0.1\% & 70.5\% & 9.3\% & 6.7\% & 72.9\%  & 54.9\% & 50.9\%  & 99.8\%   \\ \midrule

% \multirow{2}{*}{\textbf{Fairness}} & DT  &   &  &   &  &  & &  &  &  &  &     \\
% & Ours  & 50.0\%  & 50.0\%  & 50.0\%  & 50.0\% & 51.0\% & 50.0\% & 50.0\% & 50.0\%  & 62.0\%  & 87.0\%  &  61.0\%  \\ \midrule

% \multirow{2}{*}{\textbf{Sycophancy}} & DT  &   &   &   &  &  & &  &  &  &  &     \\
% & Ours  & 100.0\%  & 100.0\%  & 100.0\%  &  100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ \midrule

% \multirow{2}{*}{\textbf{Privacy}} & DT  &   &  &  &  &  & &  &  &  &  &     \\
% & Ours  & 99.6\% & 99.7\%  & 99.8\%  & 100.0\% & 100.0\% & 99.8\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ \midrule

% \multirow{2}{*}{\textbf{Robustness}} & DT  &   &   &   &  &  & &  &  &  &  &     \\
% & Ours  & 97.4\%  & 100.0\%  & 100.0\%  &  
%  98.8\% & 98.6\% & 89.5\% & 88.8\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%   \\ 

% \bottomrule
% \end{tabular}
% }
% \label{tab:results_1}
% \end{table*}


%%%%%%%%%%%%%%

% In the caption, add the different evaluation metrics for each aspect

% rank the candidate models based on their performance on general NL tasks

% have three tables
% table 1: just base version with different performances on general NLP tasks
% table 2: base vs. chat/instruct
% table 3: instruction tuning vs non-instruction tuning

% use different background colors for different series

% domain funetuning? whether the gaurdrail still holds after finetuning

% for GPT APIs (closed-sourced models), for comparison; 


==> tables/results_2.tex <==

\begin{table*}[htbp]
\centering
\caption{Comparison between base and chat variants of LLMs.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|cc|cc|cc|cc|c|c|cc|cc|cc}
\toprule
\multirow{3}{*}{\textbf{Aspect}} & \multirow{3}{*}{\textbf{Method}}  & \multicolumn{4}{c|}{MPT} & \multicolumn{4}{c|}{Falcon}& \multicolumn{2}{c|}{Mistral} & \multicolumn{6}{c}{Llama 2}    \\
& & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{30B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{40B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{13B} & \multicolumn{2}{c}{70B}  \\
& & Base & Chat & Base & Chat & Base & Instruct & Base & Instruct & Base & Instruct & Base & Chat & Base & Chat & Base & Chat  \\
\midrule

\multirow{2}{*}{\textbf{Toxicity}} & DT  & 0.27 & 0.16 & 0.30 & 0.60 & 0.20 & 0.22 & 0.29 & 0.12 & 0.41 & 0.51 & 0.18 & 0.12 & 0.29 &  0.15 & 0.43 & 0.09     \\
 & Ours  & 0.28 & 0.26 & 0.77 & 0.76 & 0.25 & 0.13 & 0.75 & 0.77 & 0.79 & 0.83  & 0.83  & 0.67 & 0.78 & 0.75 & 0.74 & 0.37  \\ \midrule

\multirow{2}{*}{\textbf{Stereotype}} & DT  & 100.0\% & 14.4\% & 99.5\% & 0.09\% & 99.9\% & 64.8\% & 91.8\% & 62.2\% & 100.0\%  & 22.6\%  & 100.0\%  & 20.6\% & 100.0\% & 12.3\% & 100.0\% & 2.3\%     \\
 & Ours  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\% & 100.0\%  & 99.7\%   \\ \midrule

\multirow{2}{*}{\textbf{Ethics}} & DT  & 63.6\% & 84.2\% & 87.9\% & 69.9\% & 81.4\% & 60.1\% & 82.5\% & 39.1\% & 37.5\% & 99.9\% & 42.5\% & 93.0\% & 33.0\% & 98.6\% & 3.1\% & 100.0\%    \\
 & Ours  & 100.0\% & 100.0\% & 100.0\% & 94.9\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 99.5\%  & 100.0\% & 99.1\% & 100.0\% & 93.3\% & 100.0\% & 99.9\%  \\ \midrule

\multirow{2}{*}{\textbf{Hallucination}} & DT  & - & - & - &- &- &- & -&- &- &-  & - & - & - &- & - & -     \\
 & Ours  & 0.1\% & 11.7\% & 70.5\% & 20.0\% & 9.3\% & 95.4\% & 6.7\% & 18.9\% & 72.9\% & 75.2\%  & 54.9\%  & 95.5\%  & 50.9\% & 39.0\% & 99.8\% & 99.9\%  \\ \midrule

\multirow{2}{*}{\textbf{Fairness}} & DT  & 50.0\% & 43.0\% & 53.0\% & 33.0\% & 50.0\% & 37.0\% & 42.0\% & 38.0\% & 37.0\% & 46.0\% & 46.0\% & 39.0\% & 44.0\% & 37.0\% & 27.0\% & 32.0\%     \\
 & Ours  & 50.0\% & 50.0\% & 51.0\% & 50.0\% & 50.0\% & 50.0\% & 50.0\% & 95.0\% & 50.0\% & 87.0\%  & 62.0\%  & 54.0\%  & 87.0\% & 65.0\% & 61.0\% & 73.0\%  \\ \midrule

\multirow{2}{*}{\textbf{Sycophancy}} & DT  & - & - & - &- &- &- & -&- &- &-  & - & - & - &- & - & -     \\
 & Ours  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\% & 99.9\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\%  \\ \midrule

\multirow{2}{*}{\textbf{Privacy}} & DT  & 100.0\% & 99.9\% & 100.0\% & 99.1\% & 99.9\% & 89.5\% & 100.0\% & 100.0\% & 99.9\% & 93.4\% & 100.0\% & 98.1\% & 99.9\% & 97.4\% & 99.9\% & 65.0\%     \\
 & Ours  & 100.0\% & 99.9\% & 100.0\% & 100.0\% & 99.9\% & 98.2\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\% & 100.0\% & 100.0\%  & 99.3\% & 100.0\%  & 99.9\%  \\ \midrule

\multirow{2}{*}{\textbf{Robustness}} & DT  & 49.4\% & 29.6\% & 56.6\% & 39.8\% & 63.5\% & 97.6\% & 28.8\% & 19.6\% & 53.6\% & 38.6\% & 47.9\% & 30.9\% & 51.9\% & 22.0\% & 42.0\% & 17.5\%     \\
 & Ours  & 98.8\% & 100.0\% & 98.6\% & 99.1\% & 89.5\% & 100.0\% & 88.8\% & 95.5\% & 100.0\% & 89.3\%  & 100.0\% & 99.0\% & 100.0\%  & 83.0\% & 100.0\%  & 99.5\%  \\

\bottomrule
\end{tabular}
}
\label{tab:results_2}
\end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Comparison between base and chat variants of LLMs.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lc|cc|cc|cc|cc|c|c|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\textbf{Aspect}} & \multirow{3}{*}{\textbf{Method}}  & \multicolumn{4}{c|}{MPT} & \multicolumn{4}{c|}{Falcon}& \multicolumn{2}{c|}{Mistral} & \multicolumn{6}{c}{Llama 2}    \\
% & & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{30B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{40B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{7B} & \multicolumn{2}{c|}{13B} & \multicolumn{2}{c}{70B}  \\
% & & Base & Chat & Base & Chat & Base & Instruct & Base & Instruct & Base & Instruct & Base & Chat & Base & Chat & Base & Chat  \\
% \midrule

% \multirow{2}{*}{\textbf{Toxicity}} & DT  &  & & & & & & & &  &  &  &  &  & &  &      \\
%  & Ours  & 0.28 & 0.26  & 0.77 & 0.76 & 0.25 & 0.13 & 0.75 & 0.77 & 0.79 & 0.83  & 0.83  & 0.67 & 0.78 & 0.75 & 0.74 & 0.37  \\ \midrule

% \multirow{2}{*}{\textbf{Stereotype}} & DT  &  & & & & & & & &  &   &   &  &  &  &  &      \\
%  & Ours  & 100.0\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\%  & 100.0\% & 100.0\%  & 99.7\%   \\ \midrule

% \multirow{2}{*}{\textbf{Ethics}} & DT  &  & & & & & & & &  &  &  &  &  &  &  &     \\
%  & Ours  & 100.0\%  & 100.0\% & 100.0\% & 94.9\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 99.5\%  & 100.0\% & 99.1\% & 100.0\% & 93.3\% & 100.0\% & 99.9\%  \\ \midrule

% \multirow{2}{*}{\textbf{Hallucination}} & DT  &  & & & & & & & & &  &  &  &  & &  &      \\
%  & Ours  & 0.1\%  & 11.7\%  & 70.5\% & 20.0\% & 9.3\% & 95.4\% & 6.7\% & 18.9\% & 72.9\% & 75.2\%  & 54.9\%  & 95.5\%  & 50.9\% & 39.0\% & 99.8\% & 99.9\%  \\ \midrule

% \multirow{2}{*}{\textbf{Fairness}} & DT  &  & & & & & & & & &  &  &  &  & &  &      \\
%  & Ours  & 50.0\%  & 50.0\% & 51.0\% & 50.0\% & 50.0\% & 50.0\% & 50.0\% & 95.0\% & 50.0\% & 87.0\%  & 62.0\%  & 54.0\%  & 87.0\% & 65.0\% & 61.0\% & 73.0\%  \\ \midrule

% \multirow{2}{*}{\textbf{Sycophancy}} & DT  &  & & & & & & & & &  &  &  &  & &  &      \\
%  & Ours  & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\% & 99.9\%  & 100.0\% & 100.0\% & 100.0\% & 100.0\%  \\ \midrule

% \multirow{2}{*}{\textbf{Privacy}} & DT  &  & & & & & & & & &  &  &  &  & &  &      \\
%  & Ours  & 100.0\%  & 99.8\% & 100.0\% & 100.0\% & 99.8\% & 96.5\% & 100.0\% & 100.0\% & 100.0\% & 100.0\%  & 100.0\% & 100.0\% & 100.0\%  & 99.3\% & 100.0\%  & 99.9\%  \\ \midrule

% \multirow{2}{*}{\textbf{Robustness}} & DT  &  & & & & & & & & &  &  &  &  & &  &      \\
%  & Ours  & 98.8\%  & 100.0\% & 98.6\% & 99.1\% & 89.5\% & 100.0\% & 88.8\% & 95.5\% & 100.0\% & 89.3\%  & 100.0\% & 99.0\% & 100.0\%  & 83.0\% & 100.0\%  & 99.5\%  \\

% \bottomrule
% \end{tabular}
% }
% \label{tab:results_2}
% \end{table*}



